MUSE: Machine Unlearning Six-Way Evaluation for Language Models

Language models (LMs) are trained on vast amounts of text data, which may include private and copyrighted content. Data owners may request the removal of their data from a trained model due to privacy or copyright concerns. However, exactly unlearning only these datapoints (i.e., retraining with the data removed) is intractable in modern-day models. This has led to the development of many approximate unlearning algorithms. The evaluation of the efficacy of these algorithms has traditionally been narrow in scope, failing to precisely quantify the success and practicality of the algorithm from the perspectives of both the model deployers and the data owners. We address this issue by proposing MUSE, a comprehensive machine unlearning evaluation benchmark that enumerates six diverse desirable properties for unlearned models: (1) no verbatim memorization, (2) no knowledge memorization, (3) no privacy leakage, (4) utility preservation on data not intended for removal, (5) scalability with respect to the size of removal requests, and (6) sustainability over sequential unlearning requests. Using these criteria, we benchmark how effectively eight popular unlearning algorithms on 7B-parameter LMs can unlearn Harry Potter books and news articles. Our results demonstrate that most algorithms can prevent verbatim memorization and knowledge memorization to varying degrees, but only one algorithm does not lead to severe privacy leakage. Furthermore, existing algorithms fail to meet deployer's expectations because they often degrade general model utility and also cannot sustainably accommodate successive unlearning requests or large-scale content removal. Our findings identify key issues with the practicality of existing unlearning algorithms on language models, and we release our benchmark to facilitate further evaluations: muse-bench.github.io

==> app/1-limitations.tex <==
\section{Limitations}

==> app/dataset_info.tex <==
% \newpage
\section{Dataset Information}
% \subsection{URL to benchmark.}

% \subsection{Dataset URLs}
% \textbf{URL to benchmark.} 

\subsection{Dataset URLs}
% \weijia{update this}
\textbf{URL to \books benchmark.} The benchmark URL can be found here: \href{https://huggingface.co/datasets/muse-bench/MUSE-Books}{link}

\textbf{URL to \books Croissant metadata.} The Croissant metadata URL can be found here: \href{https://huggingface.co/api/datasets/muse-bench/MUSE-Books/croissant}{link}

\textbf{URL to \news benchmark.} The benchmark URL can be found here: \href{https://huggingface.co/datasets/muse-bench/MUSE-News}{link}

\textbf{URL to \news Croissant metadata.} The Croissant metadata URL can be found here: \href{https://huggingface.co/api/datasets/muse-bench/MUSE-News/croissant}{link}

% The benchmark URL can be found here: \href{}{link}

% \textbf{\news metadata.} The raw for \news articles can be found on \href{https://huggingface.co/datasets/RealTimeData/bbc_latest}{HuggingFace}. We preprocess the dataset using the script provided in supplementary materials. The GPT-generated QA pairs for each article are also provided in the supplementary material. \yang{TODO: details}

% \textbf{\books metadata.} \yang{1. license for HP books? 2. shall we include HP wiki data in supp?} The GPT-generated QA pairs are also provided in the supplementary material. \weijia{link url ...}

\subsection{Author Statement \& License Information}
 We the authors bear all responsibility in case of violation of rights. We provide the license information for the data we used to construct \name:


\textbf{News.} The raw for \news articles can be found on \href{https://huggingface.co/datasets/RealTimeData/bbc_latest}{HuggingFace}.
% The data is publicly available according to its \href{https://huggingface.co/datasets/RealTimeData/bbc_latest}{HuggingFace dataset card}. 
For BBC news, all rights, including copyright, in the content of the original articles are owned by the BBC.



% and licensed under Creative Commons Attribution-ShareAlike license as follows:

%  % \weijia{bbc news is from: https://huggingface.co/datasets/RealTimeData/bbc_latest}
 
% \begin{itemize}
%     \item Content contributed before 2011-04-08 (UTC) is distributed under the terms of CC BY-SA 2.5.
%     \item Content contributed from 2011-04-08 up to but not including 2018-05-02 (UTC) is distributed under the terms of CC BY-SA 3.0.
%     \item Content contributed on or after 2018-05-02 (UTC) is distributed under the terms of CC BY-SA 4.0.
% \end{itemize}
% Please find detailed information on the license at \url{https://stats.stackexchange.com/help/licensing}.

\textbf{Books.} 
\begin{itemize}
    \item \textbf{Harry Potter Books} Acccording to JK Rowling's \href{https://www.jkrowling.com/tcs/}{Terms of Service}, Harry Potter and Fantastic Beasts characters, names and related indicia are trademarks of and © Warner Bros. Entertainment Inc.
    % all rights, including copyright, in the content of the original articles are owned by ...
    
    \item \textbf{Harry Potter FanWiki.} According to Fandom's \href{https://www.fandom.com/licensing}{Terms of Service}, the data is licensed under the Creative Commons Attribution-Share Alike License 3.0 (Unported) (CC BY-SA). 
    
\end{itemize}


\textbf{GPT-4 generated QAs for Books and News. }  The data 
is intended for research use only. 
% The dataset is distributed under the term of CC BY SA 4.0.

% \textbf{Pony.} Pony is licensed under apache-2.0 License according to its \href{https://huggingface.co/datasets/xlangai/arks_data}{HuggingFace dataset card}.

% \textbf{TheoremQA \& AoPS.} TheoremQA is licensed under MIT License according to its \href{https://huggingface.co/datasets/TIGER-Lab/TheoremQA}{HuggingFace dataset card}. AoPS does not provide license information according to its \href{https://artofproblemsolving.com/wiki/index.php/AoPS_Wiki:Copyright}{Copyright statement}. 

% \subsection{Hosting and maintenance} 





% We have a dedicated GitHub page to host the leaderboard () while data and codebase will be hosted on Huggingface (\url{https://huggingface.co/datasets/xlangai/BRIGHT}) and GitHub (\url{https://github.com/xlang-ai/bright}). We are committed to performing major maintenance on every 3-6 months.


% \newpage
\section{Data Sheet}


In addition to the data card, we follow the documentation frameworks provided by~\citet{gebru2021datasheets}.


\subsection{Motivation}

\subsubsection{For what purpose was the dataset created?}

Our dataset is designed to simulate a setting for evaluating the effectiveness of existing machine unlearning algorithms in language model applications, using representative materials such as news articles and books. The dataset and our benchmark aim to help data owners and model deployers understand the fundamental capabilities and limitations of these methods in real-world scenarios across six dimensions of machine unlearning:
\begin{enumerate}
    \item No verbatim memorization
    \item No knowledge memorization
    \item No privacy leakage
    \item Utility preservation for data not intended for removal
    \item Scalability with respect to the size of removal requests
    \item Sustainability over sequential unlearning requests
\end{enumerate}

% \subsubsection{Who created the dataset (e.g., which team, research group) and on behalf of which entity (e.g., company, institution, organization)?}

% \yang{This might be a tricky question. We can consider skipping it.}

\subsection{Composition / Collection process / Preprocessing / Cleaning}

The answers are described in our paper \Cref{app:data_details}.
% \yang{TODO: reference}.

\subsection{Distribution}

\subsubsection{Will the dataset be distributed to third parties outside of the entity (e.g., company, institution, organization) on behalf of which the dataset was created?}

No. Our dataset will be managed and maintained by the author group. %\yang{Need double-check.}

\subsubsection{How will the dataset be distributed (e.g., tarball on website, API, GitHub)?}

The evaluation dataset will be released to the public and hosted on GitHub and HuggingFace. %\yang{Need double-check}


\subsubsection{When will the dataset be distributed?}

We will release the dataset in July, 2024. %\yang{provide a time here? or upon acceptance?}.

\subsubsection{Will the dataset be distributed under a copyright or other intellectual property (IP) license, and/or under applicable terms of use (ToU)?}

Our dataset will be distributed under the
% \yang{TBD} license.
distributed under the term of CC BY SA 4.0.

% \subsubsection{Have any third parties imposed IP-based or other restrictions on
% the data associated with the instances?}

% \yang{Most of the examples we reference to skipped this question. Not sure whether we want to comment on it.}

\subsection{Maintenance}


\subsubsection{How can the owner/curator/manager of the dataset be contacted (e.g., email address)?}

Please contact Weijia Shi (\texttt{swj0419@uw.edu}) and Yangsibo Huang (\texttt{yangsibo@princeton.edu}), who are responsible for maintenance.


\subsubsection{Will the dataset be updated (e.g., to correct labeling errors, add new instances, delete instances)?}
% \begin{itemize}

Yes, if we add more data points or find any errors, we’ll update the dataset and revise the results accordingly. We'll also announce any changes on our website.
% \end{itemize}

\subsubsection{If others want to extend/augment/build on/contribute to the dataset, is there a mechanism for
them to do so?}

For dataset contributions and evaluation modifications, the most efficient way to reach us is via GitHub pull requests. For more questions, please contact Weijia Shi (\texttt{swj0419@uw.edu}), who are responsible for maintenance.

==> content/outline.tex <==
\section*{Outline}

\paragraph{Abstract + Intro$\sim$ 2 pages}: @Weijia, Figure @Yangsibo

\paragraph{(@Yangisbo) Section 2: Machine unlearning and use cases, $\sim$ 1 page} 
\begin{itemize}
    \item Background of machine unlearning  (first few work ) + rigorous mathematical formulation (forget set, retain set, heldout set, unlearned model, retrained model..)
    \item what shall we evaluate when we are evaluating machine unlearning
    \item applications: downstream tasks (privacy and copyright infringement; briefly mention what we may evaluate, with a pointer to Sec 3) 
    \item applications: how people will perform unlearning in real-world settings: 1) various forget set sizes. and 2) may be done sequentially
\end{itemize}


\paragraph{(@Weijia 3.1, @Yangsibo 3.2)Section 3: Benchmark,  $\sim$ 2 pages} 
\begin{itemize}
\item Evaluation corpus: @Weijia
- Harry Potter: orginal corpus + QA
    - forget set 
    - retain set 
- BBC: orginal corpus + QA
    - forget set 
    - retain set 
\item Evaluation Metrics @Yangsibo



\end{itemize}


\paragraph{Section 4: Method $\sim$ 1 page}



\paragraph{Experiment}  
\begin{itemize}
    \item Models and setup
    \item Expected behavior (unlearn v.s. retrain, forget v.s. heldout, infringe \& qa).. (result table: \url{https://docs.google.com/spreadsheets/d/1U99bdE-P6k_Y6sgzhYlEsvLaOUCjmF8M_w8kmwJXRXM/edit?usp=sharing})
    \item Scalability: failure cutoff size for forget size
    \item Sustainability: failure cutoff number of sequential unlearning (conditioned on a forget size)
\end{itemize}

Discuss with Chiyuan:
\begin{itemize}
    \item Discuss about the teaser figure (left: use cases; right: different evaluation aspects (Mem / MIA) + scalability / sustainability )
    \item Benchmark comparison figure (maybe combined with teaser figure) (radar plot for different methods. subplots: memorization-knowledge, memorization-verbatim, privacy, scalability, sustainability); maybe we can merge one of the radar plot into the teaser figure (better to combine with teaser figure)
    \item Main dataset figure 
    \item main table
    % \item abstract and title 
    \item per-section structure (esp how to organize results in the exp section)
\end{itemize}



% \paragraph{questions}
% \begin{itemize}
%     \item should we emphasize we focus on unlearning datasets but not behaviors
%     \item what do people think of current desirata: 
    
%     - Consistency with downstream applications (Privacy: MIA, Copyright: regurgitation)

%     - Scalability

%     - Sustainability

%     - Low side effects 

%     \item how to differentiate from TOFU: 
    
%         - TOFU only evaluates QA
    
%     \item how to differentiate from TOFU:  this paper (https://arxiv.org/pdf/2402.16835)
    
%         - only evaluate 1 model 

%         - not eval benchmark

%         - no retrained model

%     \item how much do want to say the behavior should be similar to retrained models 

%     \item emphasize unlearning a dataset or behavior
    
% \end{itemize}




% \subsection{outline}

% Machine unlearning is crucial for removing specific subsets of training data from large language models (LLMs). However, standardized methods for rigorously evaluating unlearning techniques are still lacking.  In this paper, we introduce a holistic evaluation framework called "Holistic Evaluation of Machine Unlearning" (HEMU) to profile the robustness and competitiveness of unlearning methods.

% \begin{itemize}
% \item \textbf{Taxonomy of MU application Scenarios and Metrics:} We first categorize the extensive range of potential scenarios (i.e., use cases) and metrics (i.e., desiderata, the desired behaviors for unlearning processes) relevant to LLMs.
% \item \textbf{Profiling Desired Unlearning Behavior:} We evaluate a range of unlearning methods to understand their desired behaviors and performance.
% \item \textbf{Benchmarking Across the Spectrum:} We develop a comprehensive benchmarking suite that covers the entire spectrum of evaluation metrics, allowing users to prioritize the aspects of unlearning that are most important to their specific use case.
% \end{itemize}

==> figures_latex/bbc.tex <==
\begin{wrapfigure}{r}{0.415\linewidth}
\vspace{-14mm}
\includegraphics[width=\linewidth]{figures/qa.pdf}
\vspace{-5mm}
    \caption{
    \textbf{Utility preservation vs. knowledge memorization on BBC.} $\fr$ maintains high utility on $\Dr$ while showing low knowledge memorization on $\Du$. Several unlearning methods including \GD and \NPOD, show significant utility loss. Methods like \GKL and \NPOKL, unlearn the knowledge on $\Du$ at the cost of utility.}
    \label{fig:tradeoffs}
    \vspace{-6mm}
\end{wrapfigure}
% \vspace{-3mm}

   % \GA, \NPO \GA,  \WHP,
    % An effective unlearning method should be positioned in the upper left corner, where the oracle retrained model is located. \textbf{Most unlearning methods have high forget quality, achieving effective removal but often come with significant side effects.\jz{change 'side effect'?}}%\yang{TODOs: come up with a name for the `TBD` region (any suggestions?)}

       % Utility preservation on vs. knowledge memorization on BBC. The perfect unlearned model $\fr$ has high utility preservation on $\Dr$ while low knowledge memorization on $\Du$. Many unlearning methods such as \GD, \GA, \NPO, \NPOD shows significant utilty loss, leading to 0 utility. Methods such as \GA, \GKL, \NPOK, \WHP unlearns the knwoledge on $\Du$ with utlity loss. 

==> figures_latex/privacy.tex <==
\begin{wrapfigure}{r}{0.42\linewidth}
\vspace{-3mm}
\centering
\includegraphics[width=\linewidth]{figures/auc.pdf}
\vspace{-5mm}
\caption{\textbf{ROC curves for $\Du$ vs. $\Dh$ on \news using Min-K\% Prob, with \textsf{AUC} scores in parentheses.} $\textsf{AUC}$$\approx$0.5 (i.e., $\fr$) means no significant distribution difference between two sets (i.e., no membership leakage). Most unlearning methods show under- ($\textsf{AUC}$$\ll$0.5) or over-unlearn ($\textsf{AUC}$ $\gg$0.5).
}
\label{fig:auc}
\vspace{-4mm}
\end{wrapfigure}

==> misc/checklist.tex <==
\section*{NeurIPS Paper Checklist}

%%% BEGIN INSTRUCTIONS %%%
% The checklist is designed to encourage best practices for responsible machine learning research, addressing issues of reproducibility, transparency, research ethics, and societal impact. Do not remove the checklist: {\bf The papers not including the checklist will be desk rejected.} The checklist should follow the references and precede the (optional) supplemental material.  The checklist does NOT count towards the page
% limit. 

% Please read the checklist guidelines carefully for information on how to answer these questions. For each question in the checklist:
% \begin{itemize}
%     \item You should answer \answerYes{}, \answerNo{}, or \answerNA{}.
%     \item \answerNA{} means either that the question is Not Applicable for that particular paper or the relevant information is Not Available.
%     \item Please provide a short (1–2 sentence) justification right after your answer (even for NA). 
%    % \item {\bf The papers not including the checklist will be desk rejected.}
% \end{itemize}

% {\bf The checklist answers are an integral part of your paper submission.} They are visible to the reviewers, area chairs, senior area chairs, and ethics reviewers. You will be asked to also include it (after eventual revisions) with the final version of your paper, and its final version will be published with the paper.

% The reviewers of your paper will be asked to use the checklist as one of the factors in their evaluation. While "\answerYes{}" is generally preferable to "\answerNo{}", it is perfectly acceptable to answer "\answerNo{}" provided a proper justification is given (e.g., "error bars are not reported because it would be too computationally expensive" or "we were unable to find the license for the dataset we used"). In general, answering "\answerNo{}" or "\answerNA{}" is not grounds for rejection. While the questions are phrased in a binary way, we acknowledge that the true answer is often more nuanced, so please just use your best judgment and write a justification to elaborate. All supporting evidence can appear either in the main paper or the supplemental material, provided in appendix. If you answer \answerYes{} to a question, in the justification please point to the section(s) where related material for the question can be found.

% IMPORTANT, please:
% \begin{itemize}
%     \item {\bf Delete this instruction block, but keep the section heading ``NeurIPS paper checklist"},
%     \item  {\bf Keep the checklist subsection headings, questions/answers and guidelines below.}
%     \item {\bf Do not modify the questions and only use the provided macros for your answers}.
% \end{itemize} 
 

%%% END INSTRUCTIONS %%%


\begin{enumerate}

\item {\bf Claims}
    \item[] Question: Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \item[] Answer: \answerYes{}.
    \item[] Justification: Both the abstract and introduction reflect our paper's contributions and scope.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the abstract and introduction do not include the claims made in the paper.
        \item The abstract and/or introduction should clearly state the claims made, including the contributions made in the paper and important assumptions and limitations. A No or NA answer to this question will not be perceived well by the reviewers. 
        \item The claims made should match theoretical and experimental results, and reflect how much the results can be expected to generalize to other settings. 
        \item It is fine to include aspirational goals as motivation as long as it is clear that these goals are not attained by the paper. 
    \end{itemize}

\item {\bf Limitations}
    \item[] Question: Does the paper discuss the limitations of the work performed by the authors?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We discuss the limitations of this work in \autoref{sec:conclusion}.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper has no limitation while the answer No means that the paper has limitations, but those are not discussed in the paper. 
        \item The authors are encouraged to create a separate "Limitations" section in their paper.
        \item The paper should point out any strong assumptions and how robust the results are to violations of these assumptions (e.g., independence assumptions, noiseless settings, model well-specification, asymptotic approximations only holding locally). The authors should reflect on how these assumptions might be violated in practice and what the implications would be.
        \item The authors should reflect on the scope of the claims made, e.g., if the approach was only tested on a few datasets or with a few runs. In general, empirical results often depend on implicit assumptions, which should be articulated.
        \item The authors should reflect on the factors that influence the performance of the approach. For example, a facial recognition algorithm may perform poorly when image resolution is low or images are taken in low lighting. Or a speech-to-text system might not be used reliably to provide closed captions for online lectures because it fails to handle technical jargon.
        \item The authors should discuss the computational efficiency of the proposed algorithms and how they scale with dataset size.
        \item If applicable, the authors should discuss possible limitations of their approach to address problems of privacy and fairness.
        \item While the authors might fear that complete honesty about limitations might be used by reviewers as grounds for rejection, a worse outcome might be that reviewers discover limitations that aren't acknowledged in the paper. The authors should use their best judgment and recognize that individual actions in favor of transparency play an important role in developing norms that preserve the integrity of the community. Reviewers will be specifically instructed to not penalize honesty concerning limitations.
    \end{itemize}

\item {\bf Theory Assumptions and Proofs}
    \item[] Question: For each theoretical result, does the paper provide the full set of assumptions and a complete (and correct) proof?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We do not make any theoretical claims.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include theoretical results. 
        \item All the theorems, formulas, and proofs in the paper should be numbered and cross-referenced.
        \item All assumptions should be clearly stated or referenced in the statement of any theorems.
        \item The proofs can either appear in the main paper or the supplemental material, but if they appear in the supplemental material, the authors are encouraged to provide a short proof sketch to provide intuition. 
        \item Inversely, any informal proof provided in the core of the paper should be complemented by formal proofs provided in appendix or supplemental material.
        \item Theorems and Lemmas that the proof relies upon should be properly referenced. 
    \end{itemize}

    \item {\bf Experimental Result Reproducibility}
    \item[] Question: Does the paper fully disclose all the information needed to reproduce the main experimental results of the paper to the extent that it affects the main claims and/or conclusions of the paper (regardless of whether the code and data are provided or not)?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We provide implementation details in \S\ref{sec:method} and \S\ref{sec:appendix:prompt}.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item If the paper includes experiments, a No answer to this question will not be perceived well by the reviewers: Making the paper reproducible is important, regardless of whether the code and data are provided or not.
        \item If the contribution is a dataset and/or model, the authors should describe the steps taken to make their results reproducible or verifiable. 
        \item Depending on the contribution, reproducibility can be accomplished in various ways. For example, if the contribution is a novel architecture, describing the architecture fully might suffice, or if the contribution is a specific model and empirical evaluation, it may be necessary to either make it possible for others to replicate the model with the same dataset, or provide access to the model. In general. releasing code and data is often one good way to accomplish this, but reproducibility can also be provided via detailed instructions for how to replicate the results, access to a hosted model (e.g., in the case of a large language model), releasing of a model checkpoint, or other means that are appropriate to the research performed.
        \item While NeurIPS does not require releasing code, the conference does require all submissions to provide some reasonable avenue for reproducibility, which may depend on the nature of the contribution. For example
        \begin{enumerate}
            \item If the contribution is primarily a new algorithm, the paper should make it clear how to reproduce that algorithm.
            \item If the contribution is primarily a new model architecture, the paper should describe the architecture clearly and fully.
            \item If the contribution is a new model (e.g., a large language model), then there should either be a way to access this model for reproducing the results or a way to reproduce the model (e.g., with an open-source dataset or instructions for how to construct the dataset).
            \item We recognize that reproducibility may be tricky in some cases, in which case authors are welcome to describe the particular way they provide for reproducibility. In the case of closed-source models, it may be that access to the model is limited in some way (e.g., to registered users), but it should be possible for other researchers to have some path to reproducing or verifying the results.
        \end{enumerate}
    \end{itemize}


\item {\bf Open access to data and code}
    \item[] Question: Does the paper provide open access to the data and code, with sufficient instructions to faithfully reproduce the main experimental results, as described in supplemental material?
    \item[] Answer: \answerNo{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: The dataset is accessible online. We are committed to releasing the code.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that paper does not include experiments requiring code.
        \item Please see the NeurIPS code and data submission guidelines (\url{https://nips.cc/public/guides/CodeSubmissionPolicy}) for more details.
        \item While we encourage the release of code and data, we understand that this might not be possible, so “No” is an acceptable answer. Papers cannot be rejected simply for not including code, unless this is central to the contribution (e.g., for a new open-source benchmark).
        \item The instructions should contain the exact command and environment needed to run to reproduce the results. See the NeurIPS code and data submission guidelines (\url{https://nips.cc/public/guides/CodeSubmissionPolicy}) for more details.
        \item The authors should provide instructions on data access and preparation, including how to access the raw data, preprocessed data, intermediate data, and generated data, etc.
        \item The authors should provide scripts to reproduce all experimental results for the new proposed method and baselines. If only a subset of experiments are reproducible, they should state which ones are omitted from the script and why.
        \item At submission time, to preserve anonymity, the authors should release anonymized versions (if applicable).
        \item Providing as much information as possible in supplemental material (appended to the paper) is recommended, but including URLs to data and code is permitted.
    \end{itemize}


\item {\bf Experimental Setting/Details}
    \item[] Question: Does the paper specify all the training and test details (e.g., data splits, hyperparameters, how they were chosen, type of optimizer, etc.) necessary to understand the results?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: The test details are specified in \ref{sec:appendix:dataset_stat}, \ref{sec:experiments_math} and \ref{sec:experiments_vision}.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item The experimental setting should be presented in the core of the paper to a level of detail that is necessary to appreciate the results and make sense of them.
        \item The full details can be provided either with the code, in appendix, or as supplemental material.
    \end{itemize}

\item {\bf Experiment Statistical Significance}
    \item[] Question: Does the paper report error bars suitably and correctly defined or other appropriate information about the statistical significance of the experiments?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: Since our work focus on inference of language models, the results are provided as evaluation scores on validation/test set. And we have explained how they are calculated in \ref{sec:experiments_math}.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item The authors should answer "Yes" if the results are accompanied by error bars, confidence intervals, or statistical significance tests, at least for the experiments that support the main claims of the paper.
        \item The factors of variability that the error bars are capturing should be clearly stated (for example, train/test split, initialization, random drawing of some parameter, or overall run with given experimental conditions).
        \item The method for calculating the error bars should be explained (closed form formula, call to a library function, bootstrap, etc.)
        \item The assumptions made should be given (e.g., Normally distributed errors).
        \item It should be clear whether the error bar is the standard deviation or the standard error of the mean.
        \item It is OK to report 1-sigma error bars, but one should state it. The authors should preferably report a 2-sigma error bar than state that they have a 96\% CI, if the hypothesis of Normality of errors is not verified.
        \item For asymmetric distributions, the authors should be careful not to show in tables or figures symmetric error bars that would yield results that are out of range (e.g. negative error rates).
        \item If error bars are reported in tables or plots, The authors should explain in the text how they were calculated and reference the corresponding figures or tables in the text.
    \end{itemize}

\item {\bf Experiments Compute Resources}
    \item[] Question: For each experiment, does the paper provide sufficient information on the computer resources (type of compute workers, memory, time of execution) needed to reproduce the experiments?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We provide details of computing resources like compute device, number of workers, memory and time of execution in \S\ref{sec:appendix:cost}.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item The paper should indicate the type of compute workers CPU or GPU, internal cluster, or cloud provider, including relevant memory and storage.
        \item The paper should provide the amount of compute required for each of the individual experimental runs as well as estimate the total compute. 
        \item The paper should disclose whether the full research project required more compute than the experiments reported in the paper (e.g., preliminary or failed experiments that didn't make it into the paper). 
    \end{itemize}
    
\item {\bf Code Of Ethics}
    \item[] Question: Does the research conducted in the paper conform, in every respect, with the NeurIPS Code of Ethics \url{https://neurips.cc/public/EthicsGuidelines}?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We have reviewed the NeurIPS Code of Ethics, and strictly followed it in this work.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the authors have not reviewed the NeurIPS Code of Ethics.
        \item If the authors answer No, they should explain the special circumstances that require a deviation from the Code of Ethics.
        \item The authors should make sure to preserve anonymity (e.g., if there is a special consideration due to laws or regulations in their jurisdiction).
    \end{itemize}


\item {\bf Broader Impacts}
    \item[] Question: Does the paper discuss both potential positive societal impacts and negative societal impacts of the work performed?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: Yes, we talk about boarder impacts in Appendix A.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that there is no societal impact of the work performed.
        \item If the authors answer NA or No, they should explain why their work has no societal impact or why the paper does not address societal impact.
        \item Examples of negative societal impacts include potential malicious or unintended uses (e.g., disinformation, generating fake profiles, surveillance), fairness considerations (e.g., deployment of technologies that could make decisions that unfairly impact specific groups), privacy considerations, and security considerations.
        \item The conference expects that many papers will be foundational research and not tied to particular applications, let alone deployments. However, if there is a direct path to any negative applications, the authors should point it out. For example, it is legitimate to point out that an improvement in the quality of generative models could be used to generate deepfakes for disinformation. On the other hand, it is not needed to point out that a generic algorithm for optimizing neural networks could enable people to train models that generate Deepfakes faster.
        \item The authors should consider possible harms that could arise when the technology is being used as intended and functioning correctly, harms that could arise when the technology is being used as intended but gives incorrect results, and harms following from (intentional or unintentional) misuse of the technology.
        \item If there are negative societal impacts, the authors could also discuss possible mitigation strategies (e.g., gated release of models, providing defenses in addition to attacks, mechanisms for monitoring misuse, mechanisms to monitor how a system learns from feedback over time, improving the efficiency and accessibility of ML).
    \end{itemize}
    
\item {\bf Safeguards}
    \item[] Question: Does the paper describe safeguards that have been put in place for responsible release of data or models that have a high risk for misuse (e.g., pretrained language models, image generators, or scraped datasets)?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: This paper focus on inference of language models, and thus there is no data or models to release.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper poses no such risks.
        \item Released models that have a high risk for misuse or dual-use should be released with necessary safeguards to allow for controlled use of the model, for example by requiring that users adhere to usage guidelines or restrictions to access the model or implementing safety filters. 
        \item Datasets that have been scraped from the Internet could pose safety risks. The authors should describe how they avoided releasing unsafe images.
        \item We recognize that providing effective safeguards is challenging, and many papers do not require this, but we encourage authors to take this into account and make a best faith effort.
    \end{itemize}

\item {\bf Licenses for existing assets}
    \item[] Question: Are the creators or original owners of assets (e.g., code, data, models), used in the paper, properly credited and are the license and terms of use explicitly mentioned and properly respected?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: Yes. We acknowledge the codebases we have referred to, cite and provide the urls of datasets and models in \autoref{sec:implementations}.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not use existing assets.
        \item The authors should cite the original paper that produced the code package or dataset.
        \item The authors should state which version of the asset is used and, if possible, include a URL.
        \item The name of the license (e.g., CC-BY 4.0) should be included for each asset.
        \item For scraped data from a particular source (e.g., website), the copyright and terms of service of that source should be provided.
        \item If assets are released, the license, copyright information, and terms of use in the package should be provided. For popular datasets, \url{paperswithcode.com/datasets} has curated licenses for some datasets. Their licensing guide can help determine the license of a dataset.
        \item For existing datasets that are re-packaged, both the original license and the license of the derived asset (if it has changed) should be provided.
        \item If this information is not available online, the authors are encouraged to reach out to the asset's creators.
    \end{itemize}

\item {\bf New Assets}
    \item[] Question: Are new assets introduced in the paper well documented and is the documentation provided alongside the assets?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: This paper does not release new assets.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not release new assets.
        \item Researchers should communicate the details of the dataset/code/model as part of their submissions via structured templates. This includes details about training, license, limitations, etc. 
        \item The paper should discuss whether and how consent was obtained from people whose asset is used.
        \item At submission time, remember to anonymize your assets (if applicable). You can either create an anonymized URL or include an anonymized zip file.
    \end{itemize}

\item {\bf Crowdsourcing and Research with Human Subjects}
    \item[] Question: For crowdsourcing experiments and research with human subjects, does the paper include the full text of instructions given to participants and screenshots, if applicable, as well as details about compensation (if any)? 
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: This paper does not involve crowdsourcing nor research with human subjects.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not involve crowdsourcing nor research with human subjects.
        \item Including this information in the supplemental material is fine, but if the main contribution of the paper involves human subjects, then as much detail as possible should be included in the main paper. 
        \item According to the NeurIPS Code of Ethics, workers involved in data collection, curation, or other labor should be paid at least the minimum wage in the country of the data collector. 
    \end{itemize}

\item {\bf Institutional Review Board (IRB) Approvals or Equivalent for Research with Human Subjects}
    \item[] Question: Does the paper describe potential risks incurred by study participants, whether such risks were disclosed to the subjects, and whether Institutional Review Board (IRB) approvals (or an equivalent approval/review based on the requirements of your country or institution) were obtained?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: This paper does not involve crowdsourcing nor research with human subjects.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not involve crowdsourcing nor research with human subjects.
        \item Depending on the country in which research is conducted, IRB approval (or equivalent) may be required for any human subjects research. If you obtained IRB approval, you should clearly state this in the paper. 
        \item We recognize that the procedures for this may vary significantly between institutions and locations, and we expect authors to adhere to the NeurIPS Code of Ethics and the guidelines for their institution. 
        \item For initial submissions, do not include any information that would break anonymity (if applicable), such as the institution conducting the review.
    \end{itemize}

\end{enumerate}

==> misc/checklist_data.tex <==
\section*{Checklist}

%%% BEGIN INSTRUCTIONS %%%
% The checklist follows the references.  Please
% read the checklist guidelines carefully for information on how to answer these
% questions.  For each question, change the default \answerTODO{} to \answerYes{},
% \answerNo{}, or \answerNA{}.  You are strongly encouraged to include a {\bf
% justification to your answer}, either by referencing the appropriate section of
% your paper or providing a brief inline description.  For example:
% \begin{itemize}
%   \item Did you include the license to the code and datasets? \answerYes{See Section~\ref{gen_inst}.}
%   \item Did you include the license to the code and datasets? \answerNo{The code and the data are proprietary.}
%   \item Did you include the license to the code and datasets? \answerNA{}
% \end{itemize}
% Please do not modify the questions and only use the provided macros for your
% answers.  Note that the Checklist section does not count towards the page
% limit.  In your paper, please delete this instructions block and only keep the
% Checklist section heading above along with the questions/answers below.
%%% END INSTRUCTIONS %%%

\begin{enumerate}

\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope? 
    \answerYes{See Section~\ref{sec:intro}.}
  \item Did you describe the limitations of your work?
    \answerYes{We discuss our limitations in \S\ref{sec:conclusion}.} %\yang{Subject to changes if we end up with moving them into the appendix.}
  \item Did you discuss any potential negative societal impacts of your work?
    \answerYes{We discuss broader impact of our work in \Cref{app:broader_impact}.} %\yang{Subject to changes if we end up with moving them into the appendix.}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes{We have read the ethics review guidelines and ensured that our paper conforms to them.}
\end{enumerate}

\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerNA{We don't have theoretical results.}
	\item Did you include complete proofs of all theoretical results?
    \answerNA{We don't have theoretical results.}
\end{enumerate}

\item If you ran experiments (e.g. for benchmarks)...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerYes{We provided the code and the instructions for reproducing results in the supplementary material.}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerYes{We specified training details, including model names, data splits, and hyperparameters in \S \ref{subsec:exp_setup}, with further details provided in \Cref{app:exp_setup}.}
	\item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerYes{We report standard deviation of each metric in \Cref{app:results} across all evaluated examples. Since we find the results consistent across datasets, we are not performing multiple runs for each unlearning method due to computational constraints.}
	\item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerYes{We provide the hardware configuration and typical GPU hours in \Cref{app:exp_setup}.}
\end{enumerate}

\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerYes{We cite the creators of news articles in \autoref{subsec:dataset}}
  \item Did you mention the license of the assets?
    \answerYes{We mention the data license in \autoref{app:data_details}.}
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerYes{We release the knowledge set generated by GPT-4 in \url{https://muse-bench.github.io}.} 
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerNo{We didn't collect any human data or conduct human evaluation in this work.}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
   \answerYes{See Section \ref{app:data_details}.}
\end{enumerate}

\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerNA{We did not conduct research with human subjects}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
     \answerNA{We did not conduct research with human subjects}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
     \answerNA{We did not conduct research with human subjects}
\end{enumerate}

\end{enumerate}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\iffalse
\newpage
\appendix

\section{Appendix}

Include extra information in the appendix. This section will often be part of the supplemental material. Please see the call on the NeurIPS website for links to additional guides on dataset publication.

\begin{enumerate}

\item Submission introducing new datasets must include the following in the supplementary materials:
\begin{enumerate}
  \item Dataset documentation and intended uses. Recommended documentation frameworks include datasheets for datasets, dataset nutrition labels, data statements for NLP, and accountability frameworks.
  \item URL to website/platform where the dataset/benchmark can be viewed and downloaded by the reviewers.
  \item URL to Croissant metadata record documenting the dataset/benchmark available for viewing and downloading by the reviewers. You can create your Croissant metadata using e.g. the Python library available here: https://github.com/mlcommons/croissant
  \item Author statement that they bear all responsibility in case of violation of rights, etc., and confirmation of the data license.
  \item Hosting, licensing, and maintenance plan. The choice of hosting platform is yours, as long as you ensure access to the data (possibly through a curated interface) and will provide the necessary maintenance.
\end{enumerate}

\item To ensure accessibility, the supplementary materials for datasets must include the following:
\begin{enumerate}
  \item Links to access the dataset and its metadata. This can be hidden upon submission if the dataset is not yet publicly available but must be added in the camera-ready version. In select cases, e.g when the data can only be released at a later date, this can be added afterward. Simulation environments should link to (open source) code repositories.
  \item The dataset itself should ideally use an open and widely used data format. Provide a detailed explanation on how the dataset can be read. For simulation environments, use existing frameworks or explain how they can be used.
  \item Long-term preservation: It must be clear that the dataset will be available for a long time, either by uploading to a data repository or by explaining how the authors themselves will ensure this.
  \item Explicit license: Authors must choose a license, ideally a CC license for datasets, or an open source license for code (e.g. RL environments).
  \item Add structured metadata to a dataset's meta-data page using Web standards (like schema.org and DCAT): This allows it to be discovered and organized by anyone. If you use an existing data repository, this is often done automatically.
  \item Highly recommended: a persistent dereferenceable identifier (e.g. a DOI minted by a data repository or a prefix on identifiers.org) for datasets, or a code repository (e.g. GitHub, GitLab,...) for code. If this is not possible or useful, please explain why.
\end{enumerate}

\item For benchmarks, the supplementary materials must ensure that all results are easily reproducible. Where possible, use a reproducibility framework such as the ML reproducibility checklist, or otherwise guarantee that all results can be easily reproduced, i.e. all necessary datasets, code, and evaluation procedures must be accessible and documented.

\item For papers introducing best practices in creating or curating datasets and benchmarks, the above supplementary materials are not required.
\end{enumerate}

\fi

==> tables/main2.tex <==

\begin{table}[ht]
\centering
\small
\begin{tabular}{@{}lcccc@{}}
\toprule
\textbf{Method} & \textbf{Knowledge Mem.} & \textbf{Verbatim Mem.} & \multicolumn{2}{c}{\textbf{Privacy Leakage}} \\
 & $\downarrow$ & $\downarrow$ & Over-Unlearn $\downarrow$ & Under-Unlearn $\uparrow$ \\
\midrule
\multicolumn{5}{c}{\cellcolor[HTML]{EFEFEF}\textbf{Harry Potter}} \\ 
Target        & 7 & 76 & 86 & 49 \\
Retraining     & 7 & 14 & 73 & 100 \\
\midrule
Task Vector   & 8 & 71 & 79 & 80  \\
\GA            & 0 & 0  & 75 & 74  \\
\GD           & 0 & 0  & 78 & 100 \\
\GKL           & 6 & 16 & 83 & 73  \\
\NPO           & 0 & 0  & 54 & 55  \\
\NPOD         & 0 & 0  & 58 & 96  \\
\NPOKL        & 6 & 15 & 74 & 66  \\
\WHP          & -- & -- & -- & -- \\ 
\midrule
\multicolumn{5}{c}{\cellcolor[HTML]{EFEFEF}\textbf{BBC}} \\
& \multicolumn{4}{c}{--} \\ \bottomrule
\end{tabular}
\caption{Updated table with modifications in columns and highlighting for the 'Harry Potter' dataset. The terms 'Over-Unlearning' and 'Under-Unlearning' are used to better represent the dimensions of privacy leakage. Note: '--' denotes missing data. Consider further clarifying these in the main text.}
\label{tbl:main}
\end{table}

==> tables/main_old.tex <==
\begin{table}[t]
\vspace{-8mm}
\caption{
\textbf{Most unlearning methods effectively remove verbatim and knowledge memorization but significantly impact utility and privacy.}
We evaluate the 8 algorithms described in \S\ref{sec:method} on 4 of the criteria in \name. 
We include the results of $\fr$ for reference.
%$\fr$ is the model retrained without the forget set, so it benchmarks the performance after exact unlearning. 
We highlight results in \blue{blue} if the unlearning algorithm satisfies the criterion and highlight it in \orange{orange} otherwise.
%Results in \blue{blue} indicate criteria satisfaction, while results in \orange{orange} indicate failure to meet the criteria. 
For privacy leakage, large positive values suggest ~\orange{\scriptsize \textsf{over-unlearning}}, while large negative values suggest ~\orange{\scriptsize \textsf{under-unlearning}} (see \S\ref{subsec:metric}). This table covers the results for C1 to C4, while results for C5 and C6 are shown in \Cref{fig:deployer}.
%\nascomment{red/green are bad colors to use in contrast for colorblind readers.  blue/orange tends to work better I think.} \yang{updated} 
% \nascomment{can you add the annotations to the retrain row as well?}  \yang{added}
% \nascomment{explain missing values in caption.}
% %\nascommentif time, separate the colored annotations into their own columns, and right-justify numerical columns}\yang{added} %\name. 
% %\weijia{@yangsibo, explain the color}.
% \jaechan{I'll fill in the values that are currently missing}
 % \weijia{fix for $\TV$}
% \yang{Need to mention that this table is for C1 to C4, and results for C5 and C6 are in Fig xx.}
}
\label{tbl:main}
\centering
\small
\setlength{\tabcolsep}{8pt}
\renewcommand{\arraystretch}{0.75}
\resizebox{\linewidth}{!}{
\begin{tabular}{@{}lrlrlrlrl@{}}
\toprule
 & \multicolumn{2}{c}{\scriptsize \textbf{C1. No Verbatim Mem.}} & \multicolumn{2}{c}{\scriptsize \textbf{C2. No Knowledge Mem.}} & \multicolumn{2}{c}{\scriptsize \textbf{C3. No Privacy Leak.}}  & \multicolumn{2}{c}{\scriptsize \textbf{C4. Utiltiy Preserv.}} \\
 & \multicolumn{2}{c}{\scriptsize \textsf{VerbMem} on $\Du$ ($\downarrow$)} & \multicolumn{2}{c}{\scriptsize \textsf{KnowMem} on $\Du$ ($\downarrow$)} & \multicolumn{2}{c}{\scriptsize \textsf{PrivLeak} ($\in [-5\%, 5\%]$)} & \multicolumn{2}{c}{\scriptsize \textsf{KnowMem} on $\Dr$ ($\uparrow$)} \\
% \textbf{Method} & \textbf{Knowledge} & \textbf{Verbatim} & \multicolumn{2}{c}{\textbf{Privacy Leakage}}  & \textbf{Utility Preservation} \\
 % & $\downarrow$ & $\downarrow$ & Over-Unlearn $\downarrow$ & Under-Unlearn $\uparrow$ \\
\midrule
\multicolumn{9}{c}{\cellcolor[HTML]{EFEFEF}\textbf{\news}} \\ 
Target $\ft$&
$93.3$& &
$70.2$& &
$-98.5$& &
$58.9$ \\
Retrain $\fr$&
$\mathbf{29.0}$& &
$\mathbf{33.1}$& & 
$\mathbf{0.0}$& &
$\mathbf{58.8}$ \\
\midrule
\GA&      
$0.0$& $\da{100\%}$&
$0.0$& $\da{100\%}$&
$33.8$& ~\orange{\scriptsize \textsf{over-unlearn}}&
$0.0$& $\dar{100\%}$\\
\GD&
$1.3$& $\da{95.5\%}$&
$0.0$& $\da{100\%}$&
$55.8$& ~\orange{\scriptsize \textsf{over-unlearn}}&
$0.0$& $\dar{100\%}$\\
\GKL&
$18.9$& $\da{34.8\%}$&
$41.6$& $\ua{25.7\%}$&
$-92.4$& ~\orange{\scriptsize \textsf{under-unlearn}}&
$40.1$& $\dar{31.8\%}$\\
\NPO&
$0.0$& $\da{100\%}$&
$0.0$& $\da{100\%}$&
$8.9$& ~\orange{\scriptsize \textsf{over-unlearn}}&
$0.0$& $\dar{100\%}$\\
\NPOD&
$3.2$& $\da{89.0\%}$&
$45.5$& $\ua{37.5\%}$&
$63.4$&~\orange{\scriptsize \textsf{over-unlearn}}&
$0.0$ & $\dar{100\%}$\\
\NPOKL&
$18.7$& $\da{35.5\%}$&
$45.6$& $\ua{37.8\%}$& 
$-97.5$& ~\orange{\scriptsize \textsf{under-unlearn}}&
$39.3$& $\dar{33.2\%}$\\
\TV&
$6.9$& $\da{76.2\%}$&
$64.3$& $\ua{94.3\%}$&
$1.3$& ~\blue{\scriptsize \textsf{almost no-leak}}&
$54.6$& $\dar{7.1\%}$\\
$\WHP_{\alpha=2}$&
$18.9$& $\da{34.8\%}$&
$36.9$& $\ua{11.5\%}$&
$-29.8$& ~\orange{\scriptsize \textsf{under-unlearn}}&
$47.6$& $\dar{19.0\%}$\\
\midrule
\multicolumn{9}{c}{\cellcolor[HTML]{EFEFEF}\textbf{\books}} \\
Target $\ft$&
$76.1$& &
$70.9$& &
$-65.2$& &
$79.4$\\
Retrain $\fr$&
$\mathbf{14.3}$& &
$\mathbf{27.5}$& &
$\mathbf{0.0}$& & 
$\mathbf{79.2}$\\
\midrule
\GA&      
$0.0$& $\da{100\%}$&    
$0.0$& $\da{100\%}$&    
$5.5$& ~\orange{\scriptsize \textsf{over-unlearn}}&    
$0.0$& $\dar{100\%}$\\
\GD&      
$0.0$& $\da{100\%}$&    
$0.0$& $\da{100\%}$&  
$-47.7$&~\orange{\scriptsize \textsf{under-unlearn}}&   
$0.0$& $\dar{100\%}$\\
\GKL&    
$16.1$& $\ua{12.6\%}$&   
$19.7$& $\da{28.4\%}$&
$-47.7$&~\orange{\scriptsize \textsf{under-unlearn}}&
$24.0$& $\dar{69.7\%}$\\
\NPO&
$0.0$& $\da{100\%}$&
$0.0$& $\da{100\%}$&
$12.4$&~\orange{\scriptsize \textsf{over-unlearn}}&
$0.0$& $\dar{100\%}$\\
\NPOD&
$0.0$& $\da{100\%}$&
$0.0$& $\da{100\%}$&
$-10.1$& ~\orange{\scriptsize \textsf{under-unlearn}}&
$0.0$& $\dar{57.1\%}$\\
\NPOKL&
$15.2$& $\ua{6.3\%}$&
$17.0$ & $\da{38.2\%}$&
$-19.1$& ~\orange{\scriptsize \textsf{under-unlearn}}&
$27.9$ & $\dar{27.1\%}$\\
\TV&
$70.7$& $\ua{394.4\%}$&   
$53.1$& $\ua{93.1\%}$&  
$-50.0$&~\orange{\scriptsize \textsf{under-unlearn}}&   
$65.5$& $\dar{24.2\%}$\\
\WHP&
$17.2$& $\da{20.3\%}$&
$55.2$& $\ua{100.7\%}$& 
$-14.3$& ~\orange{\scriptsize \textsf{under-unlearn}}&
$65.3$& $\dar{17.6\%}$\\
\bottomrule \\ 
\end{tabular}}

\end{table}



==> tables/notations.tex <==
\begin{wraptable}{r}{0.45\textwidth}
% \begin{table}[t]
    % \vspace{-4mm}
    \centering
    \small
    \caption{A summary of mathematical notation for machine unlearning: After unlearning, $\fu$ is expected to behave similarly to $\fr$, which is trained only on $\Dr$ but not exposed to $\Du$ during training. %\nascomment{this table is pretty redundant and the notation is not hard to understand, I suggest removing the table}
    }
    
    \label{tab:notation}
    % \small
    % \setlength{\tabcolsep}{2pt}
    \resizebox{\linewidth}{!}{
    \begin{tabular}{l|p{5cm}}
        \toprule
        \textbf{Notation} & \textbf{Description} \\
        \midrule
        $\Dt$ & Original training dataset \\

       
        
        $\Du$ & Forget set; a subset of $\Dt$ that needs to be removed \\
        
        $\Dr$ & Retain set; $\Dt\setminus\Du$ %that must be preserved in the unlearned model \chiyuan{TODO: match the definition in the text above} 
        \\
        $\Dh$ & Hold-out set; a disjoint subset of data from the same distribution of $\Dt$ \\
        \midrule
         $\mathcal{U}$ & Machine unlearning algorithm \\
         $\ft$ & Target model before unlearning \\
        $\fu$ & Unlearned model output by the unlearning algorithm
        % $\mathcal{U}(f, \Du, \Dr)$
        \\
        
        $\fr$ & Oracle model retrained on $\Dt \setminus \Du$ \\
        \bottomrule
    \end{tabular}}
    \vspace{-4mm}
% \end{table}
\end{wraptable}
